Enhancing Low-Density EEG-Based Brain-Computer Interfaces with Similarity-Keeping Knowledge Distillation

Electroencephalogram (EEG) has been one of the common neuromonitoring modalities for real-world brain-computer interfaces (BCIs) because of its non-invasiveness, low cost, and high temporal resolution. Recently, light-weight and portable EEG wearable devices based on low-density montages have increased the convenience and usability of BCI applications. However, loss of EEG decoding performance is often inevitable due to reduced number of electrodes and coverage of scalp regions of a low-density EEG montage. To address this issue, we introduce knowledge distillation (KD), a learning mechanism developed for transferring knowledge/information between neural network models, to enhance the performance of low-density EEG decoding. Our framework includes a newly proposed similarity-keeping (SK) teacher-student KD scheme that encourages a low-density EEG student model to acquire the inter-sample similarity as in a pre-trained teacher model trained on high-density EEG data. The experimental results validate that our SK-KD framework consistently improves motor-imagery EEG decoding accuracy when number of electrodes deceases for the input EEG data. For both common low-density headphone-like and headband-like montages, our method outperforms state-of-the-art KD methods across various EEG decoding model architectures. As the first KD scheme developed for enhancing EEG decoding, we foresee the proposed SK-KD framework to facilitate the practicality of low-density EEG-based BCI in real-world applications.

==> tables/4.tex <==
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{
  c| *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}
}
\toprule
\multirow{2}{*}{Teacher} 
& & {SCCNet-22} &
& & {EEGNet-22} &
& & {ShallowConvNet-22} & \\
& & 80.25 & & & 67.82 & & & 74.61 & \\
\midrule
\multirow{2}{*}{Student} 
& {SCCNet-4} & {EEGNet-4} & {ShallowConvNet-4}
& {SCCNet-4} & {EEGNet-4} & {ShallowConvNet-4} 
& {SCCNet-4} & {EEGNet-4} & {ShallowConvNet-4}\\
& 47.38 & 44.15 & 43.81 
& 47.38 & 44.15 & 43.81 
& 47.38 & 44.15 & 43.81 \\
\midrule
  KD &
  48.91 &
  \color{red} 45.69* &
  \color{red} 46.78* &
  48.93 &
  45.15 &
  \color{red} 46.76* &
  \color{red} 49.37* &
  45.37 &
  \color{red} 48.05** \\
FitNet &
  48.95 &
  \color{red} 48.37** &
  45.49 &
  47.35 &
  45.35 &
  44.93 &
  \color{blue} 45.35* &
  42.97 &
  \color{red} 47.55* \\
AT &
  47.42 &
  44.10 &
  43.64 &
  \color{red} 47.58* &
  44.07 &
  44.17 &
  47.38 &
  44.02 &
  44.10 \\
VID &
  \color{red} 48.09* &
  44.05 &
  44.75 &
  \color{red} 48.02* &
  43.82 &
  45.11 &
  \color{red} 48.03* &
  43.88 &
  45.52 \\
AB &
  \color{red} 48.66* &
  43.67 &
  42.91 &
  47.64 &
  44.28 &
  45.74 &
  46.26 &
  \color{blue} 41.82* &
  \color{red} 46.55* \\
PKT &
  \color{red} 49.09** &
  45.22 &
  \color{red} 47.09** &
  49.02 &
  \color{red} 47.00* &
  \color{red} 47.47* &
  48.35 &
  45.11 &
  \color{red} 45.54* \\
CC &
  \color{red} 49.51* &
  44.32 &
  \color{red} 47.97* &
  \color{red} 49.11* &
  44.19 &
  \color{red} \B 47.89* &
  \color{red} 49.23* &
  44.54 &
  \color{red} 47.90* \\
RKD &
  46.05 &
  44.03 &
  44.68 &
  45.85 &
  44.75 &
  44.53 &
  46.03 &
  45.10 &
  44.46 \\
SP &
  \color{red} 50.45* &
  43.82 &
  \color{red} 49.08* &
  48.01 &
  \color{red} \B 47.10* &
  46.41 &
  \B 49.49 &
  43.31 &
  47.93 \\
CRD &
  45.54 &
  \color{blue} 41.39** &
  43.81 &
  45.64 &
  43.57 &
  43.85 &
  \color{blue} 44.99* &
  \color{blue} 41.90** &
  42.79 \\ \midrule
SK &
  \color{red} 50.84** &
  \color{red} 48.44** &
  \color{red} 48.56* &
  \color{red} \B 49.61* &
  46.47 &
  \color{red} 47.69* &
  \color{red} 49.23* &
  \color{red} \B 48.40** &
  \color{red} 47.43* \\
 SK+KD &
  \color{red} \B  51.26** &
  \color{red} \B  49.35** &
  \color{red} \B  49.34** &
  49.07 &
  45.86 &
  \color{red} 47.26* &
  \color{red} \B  50.34* &
  \color{red} 48.17** &
  \color{red} \B 48.36*
  \\ \bottomrule
\end{tabular}
}



==> tables/4wKD.tex <==
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{
  c| *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}
}
\toprule
\multirow{2}{*}{Teacher} 
& & {SCCNet-22} &
& & {EEGNet-22} &
& & {ShallowConvNet-22} & \\
& & 80.25 & & & 67.82 & & & 74.61 & \\
\midrule
\multirow{2}{*}{Student} 
& {SCCNet-4} & {EEGNet-4} & {ShallowConvNet-4}
& {SCCNet-4} & {EEGNet-4} & {ShallowConvNet-4} 
& {SCCNet-4} & {EEGNet-4} & {ShallowConvNet-4}\\
& 47.38 & 44.15 & 43.81 
& 47.38 & 44.15 & 43.81 
& 47.38 & 44.15 & 43.81 \\
\midrule
  KD &
  48.91 &
  \color{red} 45.69* &
  \color{red} 46.78* &
  48.93 &
  45.15 &
  \color{red} 46.76* &
  \color{red} 49.37* &
  45.37 &
  \color{red} 48.05** \\
FitNet+KD &
  \color{red} 49.30* &
  \color{red} \B  49.67** &
  \color{red} 46.84* &
  48.65 &
  45.97 &
  45.08 &
  47.74 &
  45.97 &
  47.06 \\
AT+KD &
  48.91 &
  \color{red} 45.74* &
  \color{red} 46.79* &
  49.02 &
  45.03 &
  \color{red} 46.72* &
  \color{red} 49.38* &
  45.36 &
  \color{red} 48.03** \\
VID+KD &
  \color{red} 49.35* &
  \color{red} 45.86* &
  \color{red} 47.42** &
  48.88 &
  45.17 &
  \color{red} 47.26* &
  \color{red} 49.79* &
  45.17 &
  \color{red} 48.81** \\
AB+KD &
  \color{red} 49.83** &
  \color{red} 46.66** &
  45.51 &
  47.64 &
  44.28 &
  \color{red} 47.32* &
  \color{red} 49.37** &
  43.78 &
  \color{red} \B  49.00** \\
PKT+KD &
  \color{red} 49.85** &
  \color{red} 47.09** &
  \color{red} 47.40* &
  49.17 &
  46.81 &
  \color{red} 46.92* &
  \color{red} 49.78* &
  \color{red} 46.55** &
  \color{red} 48.54** \\
CC+KD &
  \color{red} 50.04** &
  \color{red} 45.86* &
  \color{red} 48.71** &
  48.98 &
  45.27 &
  \color{red} 47.59* &
  \color{red} 49.87* &
  \color{red} 45.72* &
  \color{red} 48.60** \\
RKD+KD &
  \color{red} 49.97* &
  \color{red} 46.27* &
  \color{red} 48.74* &
  48.47 &
  45.10 &
  \color{red} 47.92* &
  49.52 &
  44.39 &
  \color{red} 48.10* \\
SP+KD &
  \color{red} 50.74** &
  46.12 &
  \color{red} \B  49.42* &
  49.15 &
  \color{red} \B  47.15* &
  \color{red} 46.72* &
  \color{red} 50.00* &
  45.76 &
  \color{red} 48.97** \\
CRD+KD &
  48.36 &
  44.88 &
  \color{red} 46.84* &
  47.43 &
  44.98 &
  \color{red} 46.59* &
  48.96 &
  45.03 &
  \color{red} 47.33* \\ \midrule
SK &
  \color{red} 50.84** &
  \color{red} 48.44** &
  \color{red} 48.56* &
  \color{red} \B 49.61* &
  46.47 &
  \color{red} \B 47.69* &
  \color{red} 49.23* &
  \color{red} \B 48.40** &
  \color{red} 47.43* \\
SK+KD &
  \color{red} \B  51.26** &
  \color{red} 49.35** &
  \color{red} 49.34** &
  49.07 &
  45.86 &
  \color{red} 47.26* &
  \color{red} \B  50.34* &
  \color{red} 48.17** &
  \color{red} 48.36*     
  \\ \bottomrule
\end{tabular}
}



% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{
%   c| *{3}{S[table-format=-2.2,table-space-text-post=***]}|
%      *{3}{S[table-format=-2.2,table-space-text-post=***]}|
%      *{3}{S[table-format=-2.2,table-space-text-post=***]}
% }
% \multirow{2}{*}{Teacher} 
% & & {SCCNet-22} &
% & & {EEGNet-22} &
% & & {ShallowConvNet-22} & \\
% & & 80.25 & & & 67.82 & & & 74.61 & \\
% \midrule
% \multirow{2}{*}{Student} 
% & {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}
% & {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7} 
% & {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}\\
% & 47.38 & 44.15 & 43.81 
% & 47.38 & 44.15 & 43.81 
% & 47.38 & 44.15 & 43.81 \\
% \midrule
%   KD &
%   48.91 &
%   45.69* &
%   46.78* &
%   48.93 &
%   45.15 &
%   46.76* &
%   49.37* &
%   45.37 &
%   48.05** \\
% FitNet &
%   49.30* &
%   49.67** &
%   46.84* &
%   48.65 &
%   45.97 &
%   45.08 &
%   47.74 &
%   45.97 &
%   47.06 \\
% AT &
%   48.91 &
%   45.74* &
%   46.79* &
%   49.02 &
%   45.03 &
%   46.72* &
%   49.38* &
%   45.36 &
%   48.03** \\
% VID &
%   49.35* &
%   45.86* &
%   47.42** &
%   48.88 &
%   45.17 &
%   47.26* &
%   49.79* &
%   45.17 &
%   48.81** \\
% AB &
%   49.83** &
%   46.66** &
%   45.51 &
%   47.64 &
%   44.28 &
%   47.32* &
%   49.37** &
%   43.78 &
%   \B  49.00** \\
% PKT &
%   49.85** &
%   47.09** &
%   47.40* &
%   \B  49.17 &
%   46.81 &
%   46.92* &
%   49.78* &
%   46.55** &
%   48.54** \\
% CC &
%   50.04** &
%   45.86* &
%   48.71** &
%   48.98 &
%   45.27 &
%   \B  47.59* &
%   49.87* &
%   45.72* &
%   48.60** \\
% RKD &
%   49.97* &
%   46.27* &
%   48.74* &
%   48.47 &
%   45.10 &
%   47.92* &
%   49.52 &
%   44.39 &
%   48.10* \\
% SP &
%   50.74** &
%   46.12 &
%   \B  49.42* &
%   49.15 &
%   \B  47.15* &
%   46.72* &
%   50.00* &
%   45.76 &
%   48.97** \\
% CRD &
%   48.36 &
%   44.88 &
%   46.84* &
%   47.43 &
%   44.98 &
%   46.59* &
%   48.96 &
%   45.03 &
%   47.33* \\ \midrule
% Our &
%   \B  51.26** &
%   \B  49.35** &
%   49.34** &
%   49.07 &
%   45.86 &
%   47.26* &
%   \B  50.34* &
%   \B  48.17** &
%   48.36*                                         
% \end{tabular}
% }
% \label{tab:4wKD}


==> tables/7.tex <==
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{
  c| *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}
}
\toprule
\multirow{2}{*}{Teacher} 
& & {SCCNet-22} &
& & {EEGNet-22} &
& & {ShallowConvNet-22} & \\
& & 80.25 & & & 67.82 & & & 74.61 & \\
\midrule
\multirow{2}{*}{Student} 
& {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}
& {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7} 
& {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}\\
& 60.80 & 50.85 & 56.57 & 60.80 & 50.85 & 56.57 & 60.80 & 50.85 & 56.57 \\
\midrule
  KD &
  61.89 &
  \color{red} 53.43* &
  57.78 &
  60.17 &
  \color{red} 54.23* &
  55.90 &
  60.41 &
  51.43 &
  56.27 \\
FitNet &
  \color{red} 63.80* &
  \color{red} 56.94** &
  \color{blue} 49.32* &
  \color{blue} 55.81* &
  \color{red} 54.28** &
  \color{blue} 47.73* &
  \color{blue} 48.91** &
  \color{blue} 43.51* &
  \color{red} 59.78* \\
AT &
  61.28 &
  51.08 &
  56.74 &
  61.40 &
  50.90 &
  56.73 &
  61.53 &
  50.84 &
  56.73 \\
VID &
  61.96 &
  50.84 &
  57.81 &
  \color{red} 61.99* &
  50.30 &
  \color{red} 58.01* &
  \color{red} 62.33** &
  50.84 &
  \color{red} 57.95* \\
AB &
  62.05 &
  51.02 &
  \color{blue} 53.57* &
  61.04 &
  51.13 &
  56.68 &
  59.42 &
  \color{blue} 47.56** &
  57.45 \\
PKT &
  \color{red} 63.12* &
  52.99 &
  \color{red} 59.50* &
  61.92 &
  \color{red} \B 56.50* &
  58.87 &
  61.73 &
  52.65 &
  \color{red} 58.40* \\
CC &
  61.82 &
  \color{blue} 50.02* &
  57.63 &
  62.20 &
  50.80 &
  57.99 &
  61.68 &
  50.16 &
  57.62 \\
RKD &
  60.97 &
  \color{blue} 47.25* &
  57.33 &
  60.65 &
  50.36 &
  57.79 &
  57.83 &
  \color{blue} 46.60* &
  58.04 \\
SP &
  62.84 &
  49.84 &
  \color{red} 61.17* &
  \color{blue} 56.94* &
  \color{red} 56.45* &
  54.19 &
  61.45 &
  48.95 &
  58.16 \\
CRD &
  \color{blue} 55.60* &
  \color{blue} 47.41* &
  \color{blue} 50.68* &
  \color{blue} 54.43* &
  50.94 &
  \color{blue} 51.66* &
  \color{blue} 55.29** &
  \color{blue} 46.79** &
  \color{blue} 49.99* \\ \midrule
SK &
  \color{red} \B 64.25* &
  \color{red} 58.00** &
  \color{red} \B 63.13* &
  \B 62.27 &
  \color{red} 55.63* &
  \color{red} \B 60.08* &
  \B 62.38 &
  \color{red} 56.15** &
  \color{red} \B 61.18* \\
 SK+KD &
  \color{red} 64.25* &
  \color{red} \B 59.46** &
  \color{red} 62.72* &
  61.38 &
  \color{red} 55.74* &
  59.59 &
  61.87 &
  \color{red} \B 56.46* &
  59.46    
  \\ \bottomrule
\end{tabular}
}

==> tables/7wKD.tex <==
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{
  c| *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}|
     *{3}{S[table-format=-2.2,table-space-text-post=***]}
}
\toprule
\multirow{2}{*}{Teacher} 
& & {SCCNet-22} &
& & {EEGNet-22} &
& & {ShallowConvNet-22} & \\
& & 80.25 & & & 67.82 & & & 74.61 & \\
\midrule
\multirow{2}{*}{Student} 
& {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}
& {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7} 
& {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}\\
& 60.80 & 50.85 & 56.57 & 60.80 & 50.85 & 56.57 & 60.80 & 50.85 & 56.57 \\
\midrule
  KD &
  61.89 &
  \color{red} 53.43* &
  57.78 &
  60.17 &
  \color{red} 54.23* &
  55.90 &
  60.41 &
  51.43 &
  56.27 \\
FitNet+KD &
  \color{red} 63.76* &
  \color{red} 58.11** &
  52.91 &
  56.55 &
  \color{red} 55.89** &
  \color{blue} 49.47* &
  \color{blue} 53.82* &
  \color{blue} 47.70* &
  58.71 \\
AT+KD &
  61.88 &
  \color{red} 53.26* &
  57.74 &
  60.07 &
  \color{red} 54.25* &
  55.84 &
  60.42 &
  51.30 &
  56.23 \\
VID+KD &
  63.07 &
  53.27 &
  58.75 &
  60.71 &
  \color{red} 54.64* &
  55.65 &
  61.67 &
  51.93 &
  56.86 \\
AB+KD &
  62.16 &
  52.28 &
  55.71 &
  60.35 &
  \color{red} 53.94* &
  56.21 &
  59.24 &
  49.06 &
  57.62 \\
PKT+KD &
  62.32 &
  \color{red} 54.62* &
  59.21 &
  60.26 &
  \color{red} 56.57* &
  56.72 &
  60.63 &
  53.41 &
  56.84 \\
CC+KD &
  62.61 &
  \color{red} 52.99* &
  57.79 &
  60.39 &
  \color{red} 54.18* &
  54.71 &
  61.18 &
  52.08 &
  56.04 \\
RKD+KD &
  61.96 &
  52.20 &
  \color{red} 59.05* &
  61.03 &
  53.16 &
  55.76 &
  59.63 &
  51.12 &
  57.37 \\
SP+KD &
  63.23 &
  \color{red} 53.02* &
  \color{red} 60.77* &
  57.74 &
  \color{red} \B 56.70* &
  55.07 &
  61.05 &
  52.06 &
  57.61 \\
CRD+KD &
  59.56 &
  52.94 &
  54.65 &
  56.93 &
  52.39 &
  52.97 &
  \color{blue} 57.84* &
  51.51 &
  55.17 \\ \midrule
SK &
  \color{red} \B 64.25* &
  \color{red} 58.00** &
  \color{red} \B 63.13* &
  \B 62.27 &
  \color{red} 55.63* &
  \color{red} \B 60.08* &
  \B 62.38 &
  \color{red} 56.15** &
  \color{red} \B 61.18* \\
SK+KD &
  \color{red} 64.25* &
  \color{red} \B 59.46** &
  \color{red} 62.72* &
  61.38 &
  \color{red} 55.74* &
  59.59 &
  61.87 &
  \color{red} \B 56.46* &
  59.46        
  \\ \bottomrule
\end{tabular}
}


% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{
%   c| *{3}{S[table-format=-2.2,table-space-text-post=***]}|
%      *{3}{S[table-format=-2.2,table-space-text-post=***]}|
%      *{3}{S[table-format=-2.2,table-space-text-post=***]}
% }
% \multirow{2}{*}{Teacher} 
% & & {SCCNet-22} &
% & & {EEGNet-22} &
% & & {ShallowConvNet-22} & \\
% & & 80.25 & & & 67.82 & & & 74.61 & \\
% \midrule
% \multirow{2}{*}{Student} 
% & {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}
% & {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7} 
% & {SCCNet-7} & {EEGNet-7} & {ShallowConvNet-7}\\
% & 60.80 & 50.85 & 56.57 & 60.80 & 50.85 & 56.57 & 60.80 & 50.85 & 56.57 \\
% \midrule
%   KD &
%   61.89 &
%   53.43* &
%   57.78 &
%   60.17 &
%   54.23* &
%   55.90 &
%   60.41 &
%   51.43 &
%   56.27 \\
% FitNet &
%   63.76* &
%   58.11** &
%   52.91 &
%   56.55 &
%   55.89** &
%   \color{blue} 49.47* &
%   \color{blue} 53.82* &
%   \color{blue} 47.70* &
%   58.71 \\
% AT &
%   61.88 &
%   53.26* &
%   57.74 &
%   60.07 &
%   54.25* &
%   55.84 &
%   60.42 &
%   51.30 &
%   56.23 \\
% VID &
%   63.07 &
%   53.27 &
%   58.75 &
%   60.71 &
%   54.64* &
%   55.65 &
%   61.67 &
%   51.93 &
%   56.86 \\
% AB &
%   62.16 &
%   52.28 &
%   55.71 &
%   60.35 &
%   53.94* &
%   56.21 &
%   59.24 &
%   49.06 &
%   57.62 \\
% PKT &
%   62.32 &
%   54.62* &
%   59.21 &
%   60.26 &
%   56.57* &
%   56.72 &
%   60.63 &
%   53.41 &
%   56.84 \\
% CC &
%   62.61 &
%   52.99* &
%   57.79 &
%   60.39 &
%   54.18* &
%   54.71 &
%   61.18 &
%   52.08 &
%   56.04 \\
% RKD &
%   61.96 &
%   52.20 &
%   59.05* &
%   61.03 &
%   53.16 &
%   55.76 &
%   59.63 &
%   51.12 &
%   57.37 \\
% SP &
%   63.23 &
%   53.02* &
%   60.77* &
%   57.74 &
%   \B 56.70* &
%   55.07 &
%   61.05 &
%   52.06 &
%   57.61 \\
% CRD &
%   59.56 &
%   52.94 &
%   54.65 &
%   56.93 &
%   52.39 &
%   52.97 &
%   \color{blue} 57.84* &
%   51.51 &
%   55.17 \\ \midrule
% Our &
%   \B 64.25* &
%   \B 59.46** &
%   \B 62.72* &
%   \B 61.38 &
%   55.74* &
%   \B 59.59 &
%   \B 61.87 &
%   \B 56.46* &
%   \B 59.46                                           
% \end{tabular}
% }
% \label{tab:7wKD}


==> tables/UsedFeature.tex <==
\resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c}
            &  Low-level   & Medium-level& High-level  \\ \toprule
    FitNet  &              &  \checkmark &             \\ \midrule
    AT      &  \checkmark  &  \checkmark & \checkmark  \\ \midrule
    VID     &  \checkmark  &  \checkmark & \checkmark  \\ \midrule
    AB      &  \checkmark  &  \checkmark & \checkmark  \\ \midrule
    PKT     &              &             & \checkmark  \\ \midrule
    CC      &              &             & \checkmark  \\ \midrule
    RKD     &              &             & \checkmark  \\ \midrule
    SP      &              &             & \checkmark  \\ \midrule
    CRD     &              &             & \checkmark  \\ \midrule
    Ours    &              &  \checkmark & \checkmark  \\ 
    \end{tabular}}
    
